Analytical Model for IEEE 802.15.4 Multi-Hop Networks with Improved Handling of Acknowledgements and Retransmissions

The IEEE 802.15.4 standard allows for the deployment of cost-effective and energy-efficient multi-hop networks. This document features an in-depth presentation of an analytical model for assessing the performance of such networks. It considers a generic, static topology with Poisson distributed data-collection as well as data-dissemination traffic. The unslotted CSMA/CA MAC layer of IEEE 802.15.4 is closely modeled as well as an enhanced model of the neighborhood allows for consideration of collisions of packets including interferences with acknowledgements. The hidden node problem is taken into account as well as a formerly disregarded effect of repeated collisions of retransmissions. The model has been shown to be suitable to estimate the capacity of large-scale multi-hop networks.

==> setup_math.tex <==
\RequirePackage[nomain,nonumberlist]{glossaries}
\RequirePackage{xspace}
\newglossary{symbols}{sym}{sbl}{List of Symbols}

% Do not show these symbols in the List of Symbols
\newglossary{hiddensymbols}{hidsym}{hidsbl}{} 

% Parameters:
% 1: name of the command
% 2: sort key 
% 3: symbol in math mode
% 4: description
\newcommand{\sym}[4]{\newglossaryentry{#1}{type=symbols,
        sort=#2,
        name={\ensuremath{#3}\xspace},
        description={#4}}%
    \expandafter\newcommand\expandafter{\csname #1\endcsname}{\gls{#1}}%
}

% Parameters:
% 1: name of the command
% 2: sort key 
% 3: symbol in math mode
% 4: description
\newcommand{\symHidden}[4]{\newglossaryentry{#1}{type=hiddensymbols,
        sort=#2,
        name={\ensuremath{#3}\xspace},
        description={#4}}%
    \expandafter\newcommand\expandafter{\csname #1\endcsname}{\gls{#1}}%
}

% Parameters:
% 1: name of the command
% 2: is concatinated to the name for the default value
% 3: sort key
% 4: symbol in math mode
% 5: default parameter in math mode
% 6: description
\newcommand{\symLower}[6]{\newglossaryentry{#1#2}{type=symbols,
        sort=#3,
        text={\ensuremath{#4}\xspace},
        name={\ensuremath{#4_{#5}}\xspace},
        description={#6}}%
    \expandafter\newcommand\expandafter{\csname #1\endcsname}[1]{\ensuremath{\gls{#1#2}_{##1}}}%
    \expandafter\newcommand\expandafter{\csname #1#2\endcsname}{\ensuremath{\gls{#1#2}_{#5}}}%
}

% Parameters:
% 1: name of the command
% 2: is concatinated to the name for the default value (and for the sort key)
% 3: symbol in math mode
% 4: symbol in math mode before the comma in the lower place
% 5: default parameter in math mode
% 6: description
\newcommand{\symLowerComma}[6]{\newglossaryentry{#1#2}{type=symbols,
        sort=#1#2,
        text={\ensuremath{#3}\xspace},
        name={\ensuremath{#3_{#4,#5}}\xspace},
        description={#6}}%
    \expandafter\newcommand\expandafter{\csname #1\endcsname}[1]{\gls{#1#2}_{#4,##1}}%
    \expandafter\newcommand\expandafter{\csname #1#2\endcsname}{\gls{#1#2}_{#4,#5}}%
}

% Parameters:
% 1: name of the command
% 2: is concatinated to the name for the default value
% 3: sort key
% 4: symbol in math mode
% 5: default parameter in math mode
% 6: description
\newcommand{\symFun}[6]{\newglossaryentry{#1#2}{type=symbols,
        sort=#3,
        text={\ensuremath{#4}\xspace},
        name={\ensuremath{#4\left({#5}\right)}\xspace},
        description={#6}}%
        \expandafter\newcommand\expandafter{\csname #1\endcsname}[1]{\gls{#1#2}\left({##1}\right)}%
        \expandafter\newcommand\expandafter{\csname #1#2\endcsname}{\gls{#1#2}\left({#5}\right)}%
}

\newcommand{\stdname}[1]{{\it #1}}
\newcommand{\relation}[2]{\left\{\left(#1\right) \,|\, #2 \right\}}
\newcommand{\linkset}[2]{\left\{#1 \,|\, #2 \right\}}

\sym{pgenup}    {gnu}{g_{\text{up}}}{Packet generation rate in upstream}
\sym{pgendown}  {gnd}{g_{\text{down}}}{Packet generation rate in downstream}
\sym{Iup}       {Iup}{I_{\text{up}}}{Packet interval in upstream}
\sym{Idown}     {Idown}{I_{\text{down}}}{Packet interval in downstream}
\sym{rootnode}  {r}{r}{The gateway node}
\sym{LenSuccess}{Ls}{L_s}{Total time for a successful transmission}
\sym{LenFail}   {Lc}{L_c}{Total time for an unsuccessful transmission}
\symLower{W}{i} {Wi}{W}{i}{Maximum backoff time span for the $i^{\text{th}}$ channel sensing}

\symLower{R}{l} {Rl}{R}{l}{Reliability of packet transmission on a link}
\sym{Rlconst}       {Rlindep}{R_{l,indep}}{Reliability of a link assuming constant collision probability over $j$}
\symLowerComma{Rup}{n}{\mathfrak{R}}{\text{up}}{l}{Reliability that a packet sent by $n$ arrives at the gateway}
\symLowerComma{Rdown}{n}{\mathfrak{R}}{\text{down}}{l}{Reliability that a packet sent by the gateway arrives at $n$}

\symHidden{sublinks}{}{{\bf S}}{}
\symHidden{tree}{T}{\mathcal{T}}{}

\symFun{inrange}{vw}{D}{\ensuremath{D}}{v,w}{Predicate that describes potential collisions between nodes}

\sym{Prx}       {Prx}{P_{rx}}{Reception power}
\sym{Ptx}       {Ptx}{P_{tx}}{Transmission power}
\sym{PN}        {PN}{P_{N}}{Noise power}
\sym{Pdist}     {Pdist}{P_{dist}}{Minimum power that interfers with a reception}
\symLower{SNR}{l}{SNRl}{\text{SNR}}{l}{Signal to noise ratio}
\symLower{BER}{l}{BERl}{\text{BER}}{l}{Bit error rate}
\symLower{PER}{bl}{PERbl}{\text{PER}}{b,l}{Packet error rate for a transmission of $b$ bytes}
\symFun{T}{pc}{Tpc}{T}{p,c}{$p$ is parent of $c$ in the routing tree}

\let\L\undefined
\sym{L}		{L}{{\bf L}}{The set of active links}
\sym{Lup}	{Lup}{{\bf L}_{\text{up}}}{The set of active links in upstream direction}
\sym{Ldown}	{Ldown}{{\bf L}_{\text{down}}}{The set of active links in downstream direction}

\let\SS\undefined
\symLowerComma{SS}{l}{\mathcal{S}}{\mathcal{S}}{l}{Set of links with senders in the interference range of the sender}
\symLowerComma{RS}{l}{\mathcal{R}}{\mathcal{S}}{l}{Set of links with senders in the interference range of the receiver}
\symLowerComma{SR}{l}{\mathcal{S}}{\mathcal{R}}{l}{Set of links with receivers in the interference range of the sender}
\symLowerComma{RR}{l}{\mathcal{R}}{\mathcal{R}}{l}{Set of links with receivers in the interference range of the receiver}

\symFun{Q}{tS}{Qts}{Q}{t,\sublinks}{Probability that at least one link in \sublinks starts a transmission within $t$ time units}
\newcommand{\someoccupy}[2]{\Q{#1, #2}}
\newcommand{\somesending}[1]{\someoccupy{1}{#1}}

% Events
\newcommand{\Prob}[1]{P\left(#1\right)}
\symLower{collpacket}{l}    {CPl}{\mathcal{C\hspace{-0.2em}P}}{l}{Event that a packet on $l$ collides}
\symLower{collack}{l}       {CAl}{\mathcal{C\hspace{-0.2em}A}}{l}{Event that an acknowledgement on $l$ collides}
\symLower{collmut}{l}       {CBl}{\mathcal{C\hspace{-0.1em}B}}{l}{Event that transmissions mutually collide}
\symLower{collrepeat}{l}    {CRl}{\mathcal{C\hspace{-0.2em}R}}{l}{Event that transmissions collide again}
\symLower{lostpacket}{l}    {LPl}{\mathcal{L\hspace{-0.1em}P}}{l}{Event that a packet on $l$ gets lost}
\symLower{lostack}{l}       {LAl}{\mathcal{L\hspace{-0.1em}A}}{l}{Event that an acknowledgement on $l$ gets lost}
\newcommand{\pnsp}[1]{\Prob{\collpacket{l,#1}}}
\newcommand{\pnsack}[1]{\Prob{\collack{l,#1}}}
\newcommand{\pnsb}[1]{\Prob{\collmut{l,#1}}}

\sym{Pnoack}  {Pnoack}{P_{\text{noACK},l}}{Probability that no acknowledgement arrives after sending a packet over $l$}

\newcommand{\bothset}{\collmut{l,2}}
\newcommand{\bothsameset}{\collmut{l,1}}

\newcommand{\bc}[1]{{\collrepeat{l,2}}^{#1}}
\newcommand{\bsc}[1]{{\collrepeat{l,1}}^{#1}}

\symLower{pdesc}{n}         {gn}{\gamma}{n}{Number of proper descendants of node $n$}

\symLower{rstate}{s}        {kn}{\kappa}{s}{State in the retransmission Markov chain}
\newcommand{\rstcf}{\rstate{cf} }
\newcommand{\rstsucc}{\rstate{succ} }

\symLower{mstate}{s}        {tn}{\theta}{s}{State in the MAC layer Markov chain}

\newcommand{\mtr}[2]{P\left(#1 \to #2\right)}
\newcommand{\mmtr}[2]{\mtr{\mstate{#1}}{\mstate{#2}}}

\sym{maxbackoffs}   {m}{m}{Maximum number of channel sensing attempts (\stdname{macMaxCSMABackoffs})}
\sym{initbexp}      {m0}{m_0}{Initial backoff exponent}
\sym{maxbexp}       {mb}{m_b}{Maximum backoff exponent}
\newcommand{\mb}{\maxbexp}
\sym{mo}            {mo}{\overline{m}}{Shortcut for $\maxbexp - \initbexp$}
\sym{maxretrans}    {n}{n}{Maximum number of retransmission attempts (\stdname{macMaxFrameRetries})}
\sym{Len}           {L}{L_p}{Duration of packet sending} % TODO no L or harmonize with L set!!!
\sym{BytesPacket}   {B}{B}{Bytes per packet} % TODO no L or harmonize with L set!!!
\sym{IFS}           {IFS}{IFS}{Inter-frame spacing as defined in the standard}
\sym{BytesACK}      {Back}{B_{\mbox{\tiny ACK}}}{Bytes per acknowledgement} % TODO no L or harmonize with L set!!!
\sym{Lack}          {Lack}{L_{\mbox{\tiny ACK}}}{Duration of acknowledgement}
\sym{Sb}            {Sb}{S_b}{Backoff unit time (used as basic time unit)}

\symLower{linkrate}{l}  {ll}{\lambda}{l}{Packet sending rate}
%\newcommand{\linkrate}[1]{\lambda_{#1}}
%\sym{linkratel}     {l}{\linkrate{l}}{Packet sending rate}
\symLower{Psend}{l}     {ql}{q}{l}{Packet sending probability}
\newcommand{\ql}{\Psendl}
%\newcommand{\Psend}[1]{q_{#1}}
%\sym{Psendl}        {ql}{\Psend{l}}{Packet sending probability}
\symLower{forwarded}{l}{mul}{\mu}{l}{Packet forwarding rate}
%\newcommand{\forwarded}[1]{\mu_{#1}}
%\sym{forwardedl}    {mu}{\forwarded{l}}{Packet forwarding rate}

\sym{yl}            {yl}{y_l}{Shortcut for $\Pnoack \cdot \left(1-{\al}^{\maxbackoffs+1}\right)$}
\sym{bl}            {bl}{\beta_l}{Shortcut for $1 - {\al}^{\maxbackoffs+1}$}

\sym{tack}          {tack}{t_{ack}}{Time interval between packet transmission and acknowledgement}
\sym{tmACK}         {tmack}{t_{m,ack}}{Time to wait for a lost acknowledgement (\stdname{macAckWaitDuration})}

\let\a\undefined
\symLower{a}{l}     {al}{\alpha}{l}{Probability of sensing a busy channel}
\let\t\undefined
\symLower{t}{l}     {tl}{\tau}{l}{Probability of a channel sensing attempt}
\sym{apkt}          {alaapkt}{\a{pkt,l}}{Probability of sensing a packet}
\sym{aack}          {alack}{\a{ack,l}}{Probability of sensing an acknowledgement}
\sym{Nodes}         {N}{N}{Total number of nodes in the network}

\symLower{stat}{zeta}{b}{b}{\zeta}{Probability of being in state $\mstate{\zeta}$}


